The Fast Cauchy Transform and Faster Robust Linear Regression

We provide fast algorithms for overconstrained $\ell_p$ regression and related problems: for an $n\times d$ input matrix $A$ and vector $b\in\mathbb{R}^n$, in $O(nd\log n)$ time we reduce the problem $\min_{x\in\mathbb{R}^d} \|Ax-b\|_p$ to the same problem with input matrix $\tilde A$ of dimension $s \times d$ and corresponding $\tilde b$ of dimension $s\times 1$. Here, $\tilde A$ and $\tilde b$ are a coreset for the problem, consisting of sampled and rescaled rows of $A$ and $b$; and $s$ is independent of $n$ and polynomial in $d$. Our results improve on the best previous algorithms when $n\gg d$, for all $p\in[1,\infty)$ except $p=2$. We also provide a suite of improved results for finding well-conditioned bases via ellipsoidal rounding, illustrating tradeoffs between running time and conditioning quality, including a one-pass conditioning algorithm for general $\ell_p$ problems. We also provide an empirical evaluation of implementations of our algorithms for $p=1$, comparing them with related algorithms. Our empirical results show that, in the asymptotic regime, the theory is a very good guide to the practical performance of these algorithms. Our algorithms use our faster constructions of well-conditioned bases for $\ell_p$ spaces and, for $p=1$, a fast subspace embedding of independent interest that we call the Fast Cauchy Transform: a distribution over matrices $\Pi:\mathbb{R}^n\mapsto \mathbb{R}^{O(d\log d)}$, found obliviously to $A$, that approximately preserves the $\ell_1$ norms: that is, with large probability, simultaneously for all $x$, $\|Ax\|_1 \approx \|\Pi Ax\|_1$, with distortion $O(d^{2+\eta})$, for an arbitrarily small constant $\eta>0$; and, moreover, $\Pi A$ can be computed in $O(nd\log d)$ time. The techniques underlying our Fast Cauchy Transform include fast Johnson-Lindenstrauss transforms, low-coherence matrices, and rescaling by Cauchy random variables.

==> alg-LpCond1.tex <==

\begin{figure}[t]
\begin{center}
%%% CHANGE FOR SODA %%% 
\framebox[6.4in]{\parbox{6.2in}{
%%% \framebox[3.3in]{\parbox{3.1in}{
\textsf{OnePassConditioning}$(A,p)$:
\begin{algorithmic}[1]
   \STATE 
   Partition $A$ along its rows into sub-matrices of size 
   $d^2 \times d$, denoted by $A_1, \ldots, A_M$.
   \STATE 
   For each $A_i$, compute its economy-sized SVD: $A_i = U_i \Sigma_i V_i^T$.
   \STATE 
   Let $\tilde{A}_i = \Sigma_i V_i^T$ for $i=1,\ldots,M$,
   \begin{equation*}
   \tilde{\mathcal{C}} = \{ x \,|\, \left(\sum_{i=1}^M \|\tilde{A}_i x\|_2^p\right)^{1/p} \leq
    1\}, \text{ and } \tilde{A} = {\tiny \begin{pmatrix} \tilde{A}_1 \\
        \vdots \\ \tilde{A}_M
        \end{pmatrix}}.
    \end{equation*}
   \STATE 
   Compute $\tilde{A}$'s SVD: $\tilde{A} = \tilde{U}\tilde{\Sigma}\tilde{V}^T$.
   \STATE 
   Let $\mathcal{E}_0 = \mathcal{E}(0, E_0)$ where 
   $E_0 = d^{1/p-1/2} \tilde{V} \tilde{\Sigma}^{-1}$;
   and note that $\mathcal{E}_0$ gives an $(M d^2)^{1/p-1/2}$-rounding of 
   $\tilde{\mathcal{C}}$.
   \STATE 
   Compute an ellipsoid $\mathcal{E} = \mathcal{E}(0, E)$ that gives a
   $2d$-rounding of $\tilde{\mathcal{C}}$. 
   \STATE
   Return $E$.
\end{algorithmic}
}}
\end{center}
\caption{A one-pass algorithm for finding an $\ell_p$ well-conditioned basis 
of an $n \times d$ matrix $A$.}
\label{alg:l1_cond}
\end{figure}


==> alg-LpCond2.tex <==

\begin{figure}[t]
\begin{center}
%%% CHANGE FOR SODA %%% 
\framebox[6.4in]{\parbox{6.2in}{
%%% \framebox[3.3in]{\parbox{3.1in}{
\textsf{FasterOnePassConditioning}$(A,p)$:
\begin{algorithmic}[1]
   \STATE 
   Partition $A$ along its rows into sub-matrices of size 
   $O(d^3 \log d)\times d$, denoted by $A_1, \ldots, A_M$.
   \STATE 
   For each $A_i$, compute 
   $\tilde{A}_i = \text{FJLT}(A_i) \in \mathbb{R}^{O(d \log d) \times d}$.
   \STATE 
   Let 
   \begin{equation*}
   \tilde{\mathcal{C}} = \{ x \,|\, \left(\sum_{i=1}^M \|\tilde{A}_i x\|_2^p\right)^{1/p} \leq
   1\}, \text{ and } \tilde{A} = {\tiny \begin{pmatrix} \tilde{A}_1 \\
       \vdots \\ \tilde{A}_M
       \end{pmatrix}}.
   \end{equation*}
   \STATE 
   Compute an ellipsoid $\mathcal{E} = \mathcal{E}(0, E)$ that gives a
   $2d$-rounding of $\tilde{\mathcal{C}}$. 
   \STATE
   Return $E$.
\end{algorithmic}
}}
\end{center}
\caption{A faster one-pass algorithm for finding an $\ell_p$ 
well-conditioned basis of an $n \times d$ matrix $A$.}
\label{alg:l1_cond_fast}
\end{figure}


==> appdx-pfLp.tex <==
\section{Proof of Theorem~\ref{thm:basisLp} (Fast $\ell_p$ Well-conditioned Basis)}
%%%\begin{proof} (of Theorem~\ref{thm:basisLp}.)
\label{sxn:app-pfbasisLp}

Recall that $y = Ax$ and
write $y^T = [z_1^T, z_2^T, \ldots, z_{n/t}^T]$. Set
\math{s=36(k+\frac{8d}{c_3\eps}+\log (2c_1))/c_2\eps^2}. Applying 
Lemma~\ref{thm:subspace} with \math{\eps=\frac12}, 
for all $x \in \mathbb{R}^d$,
 and any particular $i \in [n/t]$, the inequalities
\mld{
\sqrt{\textstyle\frac12}\norm{z_i}_2\le\norm{Gz_i}_2\le
\sqrt{\textstyle\frac32}\norm{z_i}_2\label{eq:appLp1}
}
hold with probability at least \math{1-e^{-k}}.
Using 
a union bound, the same inequalities hold for all $i \in [n/t]$
with probability at least $1-(n/t)e^{-k}$. All the following results
assume \r{eq:appLp1} to hold, and hence are valid with 
probability at least $1-(n/t)e^{-k}$.

\begin{lemma}\label{lem:appLp1}
\mand{
\begin{array}{l@{\hspace*{0.25in}}l}
\text{For \math{1\le p\le 2},}&
 t^{1/2-1/p}\sqrt{\textstyle\frac12}\norm{z_i}_p\le\norm{Gz_i}_p\le
 s^{1/p-1/2} \sqrt{\textstyle\frac32} \norm{z_i}_p;\\[10pt]
\text{For \math{2<p},}&
s^{1/p-1/2} \sqrt{\textstyle\frac12}  \norm{z_i}_p\le\norm{Gz_i}_p\le
t^{1/2 - 1/p}\sqrt{\textstyle\frac32}  \norm{z_i}_p
\end{array}
}
\end{lemma}
\begin{proof}
Let \math{0<p\le q} and \math{x\in\R^{m}} be arbitrary. Then,
\mld{
\norm{x}_q\le\norm{x}_p\le m^{1/p-1/q}\norm{x}_q.\label{eq:appLp2}
}
In \r{eq:appLp2}, the latter inequality is equivalent to 
H\:{o}lder's inequaltiy and the former follows by elementary calculus.
Recall that \math{z_i\in\R^t} and \math{Gz_i\in\R^s}.
Combining \r{eq:appLp1} and \r{eq:appLp2},  for $1\le p \leq 2$, we upper
bound \math{\norm{Gz_i}_p} as follows:
$$\norm{Gz_i}_p
	\le s^{1/p-1/2}\norm{Gz_i}_2
	\le s^{1/p-1/2} \sqrt{\textstyle\frac32} \norm{z_i}_2
	\le s^{1/p-1/2} \sqrt{\textstyle\frac32} \norm{z_i}_p,$$
Similarly, for $1\le p \leq 2$, we lower
bound \math{\norm{Gz_i}_p} as follows:
$$\norm{Gz_i}_p
	\ge \norm{Gz_i}_2
	\ge \sqrt{\textstyle\frac12}\norm{z_i}_2
	\ge \sqrt{\textstyle\frac12} t^{1/2-1/p}\norm{z_i}_p.
$$
An analogous derivation for  $p > 2$ gives
\eqan{
&\norm{Gz_i}_p
	\le \norm{Gz_i}_2
	\le \sqrt{\textstyle\frac32} \norm{z_i}_2
	\le \sqrt{\textstyle\frac32} t^{1/2 - 1/p} \norm{z_i}_p,&\\
&
\norm{Gz_i}_p
	\ge s^{1/p-1/2}\norm{Gz_i}_2
	\ge s^{1/p-1/2} \sqrt{\textstyle\frac12} \norm{z_i}_2
 	\ge s^{1/p-1/2} \sqrt{\textstyle\frac12}  \norm{z_i}_p.
&
}
\end{proof}
We now give the result which is an analog of the FCT2 low
distortion embedding result for \math{\ell_p}.
\begin{lemma}[Low distortion]\label{lem:appLp2}
For any \math{x\in\R^d},
\mand{
\norm{Ax}_p \le \gamma \norm{FAx}_p \le \sqrt{3} (st)^{|1/p-1/2|}\norm{Ax}_p,
}
where \math{\gamma=t^{1/p-1/2}\sqrt{2}} for \math{p\in[1,2]} and
\math{\gamma=s^{1/2-1/p}\sqrt{2}} for \math{2<p}.
\end{lemma}
\begin{proof}
The lemma follows from 
Lemma~\ref{lem:appLp2}. First raise the inequalities in 
 Lemma~\ref{lem:appLp2} to the power 
\math{p}; second, summing over \math{i} and observe that 
$\norm{Ax}_p^p = \norm{y}_p^p = \sum_i \norm{z_i}^p$
and $\norm{FAx}_p^p = \sum_i \norm{Gz_i}_p^p$.
\end{proof}
\remove{
Since $\norm{Ax}_p^p = \norm{y}_p^p = \sum_i \norm{z_i}^p$
and $\norm{FAx}_p^p = \sum_i \norm{Gz_i}_p^p$,
for $p\in [1,2]$ we have with probability $1-1/n$
\[
\sqrt{\textstyle\frac12} t^{1/2-1/p}\norm{Ax}_p
	\le \norm{FAx}_p \le \sqrt{\textstyle\frac32} s^{1/p-1/2} \norm{Ax}_p,
\]
and for $p\in [2,\infty)$ with probability $1-1/n$
\[
\sqrt{\textstyle\frac12} s^{1/p-1/2} \norm{Ax}_p
	\le \norm{FAx}_p \le \sqrt{\textstyle\frac32} t^{1/2 - 1/p} \norm{Ax}_p.
\]
In either case,
\begin{equation}\label{eqn:first}
\norm{Ax}_p \le \gamma_p \norm{FAx}_p \le \sqrt{3} (st)^{|1/p-1/2|}\norm{Ax}_p.
\end{equation}
}

We are now ready to analyze Algorithm~\ref{alg:basisLp}.
Theorem \ref{thm:basisOld} provides us with a change of basis 
matrix \math{\Gamma} which guarantees that 
\math{FA\Gamma} is $(\alpha,\beta,p)$-well-conditioned, where 
\math{\alpha} and \math{\beta} depend on \math{d} and \math{p},
 and are given in 
Theorem \ref{thm:basisOld}.
Therefore, \math{
\|FA \Gamma \|_p \leq \alpha 
}
and for all $x \in \mathbb{R}^d$,
\math{
\|x\|_q \leq \beta \|FA\Gamma x\|_p.
}
We now analyze \math{A\Gamma}.
\mand{
\norm{A\Gamma}_p^p
=\sum_i \|A \Gamma_i \|_p^p
\mathop{\buildrel (a)\over\le}\sum_i \gamma^p\|FA \Gamma_i \|_p^p
=\gamma^p\sum_i \|FA \Gamma \|_p^p
\mathop{\buildrel (b)\over\le}\gamma^p\alpha^p,
}
where (a) follows from Lemma~\ref{lem:appLp2} and (b) from the conditioning
of \math{FA\Gamma}. 
Raising both sides to the power \math{1/p} we have
\math{\norm{A\Gamma}_p\le\gamma\alpha}, or that \math{\norm{A\Gamma/\gamma}_p
\le\alpha}.
Now consider any $x \in \mathbb{R}^d$.
\mand{
\|x\|_q
\mathop{\buildrel (a)\over\le}
\beta \|F A \Gamma x\|_p
\mathop{\buildrel (b)\over\le}
\frac\beta\gamma\sqrt{3} (st)^{|1/p-1/2|} \|A \Gamma x\|_p
=
\beta\sqrt{3} (st)^{|1/p-1/2|}\|(A \Gamma/\gamma)  x\|_p
}
Hence $A \Gamma/\gamma$ is an 
$(\alpha, \beta \sqrt{3} (st)^{|1/p-1/2|} , p)$-well-conditioned
basis. The probability of succes is at least \math{1-(n/t)e^{-k}\ge 1-1/n} by
choosing \math{k>2\log n}. This means that 
\math{s=\Theta(d+\log n)} as is the case in the construction of \math{F}.
Plugging in the values of \math{\alpha} and \math{\beta} from 
Theorem~\ref{thm:basisOld} gives the result.

\paragraph{Running Time.}
The time to compute
$F A$ is $O(nd \log d)$.  The dimensions
of  $FA$ are \math{ns/t\times d=ns/(sd^4)\times d=n/d^4\times d}. Thus,
 the running
time (from Theorem~\ref{thm:basisOld}) to compute 
the change of basis \math{\Gamma} is \math{O((n/d^4)d^5\log n)=O(nd\log n)}.

 $O(n/d^4) \times d$. the time to
compute $\Gamma$ from $F A$ is $O(nd \log n)$. 
%%%\end{proof}



==> resultsLpXM.tex <==
%% NO CALL NOW %% 
%% NO CALL NOW %% \section{Additional Improvements for Rounding and Conditioning in $\ell_p$}
%% NO CALL NOW %% \label{sxn:extensionlpXM}
%% NO CALL NOW %% 
%% NO CALL NOW %% In this section, we describe several additional improvements for finding good
%% NO CALL NOW %% bases in $\ell_p$, which, when combined with our results from previous sections,
%% NO CALL NOW %% lead to still further improvements for $\ell_1$ and $\ell_p$ regression
%% NO CALL NOW %% problems.  After some preliminary discussion setting notation for these more
%% NO CALL NOW %% general methods, we will present in Section~\ref{sxn:extensionlpXM-rounding} our
%% NO CALL NOW %% improved results for ellipsoidal rounding, and we will then in
%% NO CALL NOW %% Section~\ref{sxn:extensionlpXM-onepasscond} use this result to derived improved
%% NO CALL NOW %% bounds for ``one-pass conditioning.''
%% NO CALL NOW %% 
%% NO CALL NOW %% The methods of this section complement the FCT-based methods in the sense that
%% NO CALL NOW %% the FCT may be viewed as a tool to compute a good basis, and the ellipsoid-based
%% NO CALL NOW %% methods of this section provide an alternate way to compute a good basis.  
%% NO CALL NOW %% FCT1 and FCT2 are independent of $A$ and require very little offline
%% NO CALL NOW %% work, but there are two aspects of them that motivate the rounding and
%% NO CALL NOW %% conditioning approach of this section.  First, the constants hidden in the ``big
%% NO CALL NOW %% O'' in Theorems~\ref{theorem:FCT2} and~\ref{theorem:FCT} are not explicitly
%% NO CALL NOW %% given, and they may be too large for practical use, especially when $d$ is
%% NO CALL NOW %% small. Second, the FCT-based methods are randomized algorithms that fail with
%% NO CALL NOW %% certain probability.  We can always repeat trials to make the failure rate
%% NO CALL NOW %% arbitrarily small, but we don't have a simple way to check whether a trial
%% NO CALL NOW %% succeeds or not.
%% NO CALL NOW %% 
%% NO CALL NOW %% % To state our rounding and conditioning algorithms, we will use an equivalent 
%% NO CALL NOW %% % formulation of the $\ell_p$ regression Problem~\eqref{eq:lp_reg} that 
%% NO CALL NOW %% % consists of a homogeneous objective function and an affine constraint:
%% NO CALL NOW %% % \begin{equation}
%% NO CALL NOW %% %   \label{eq:lp_reg_homog}
%% NO CALL NOW %% %   \begin{aligned}
%% NO CALL NOW %% %     & \text{minimize}_{x \in \mathbb{R}^d} && \|A x\|_p \\
%% NO CALL NOW %% %     & \text{subject to} && c^T x = 1.
%% NO CALL NOW %% %   \end{aligned}
%% NO CALL NOW %% % \end{equation}
%% NO CALL NOW %% % (Thus, in this section, the matrix $A$ refers to the $A$ of 
%% NO CALL NOW %% % (\ref{eq:lp_reg_homog}).
%% NO CALL NOW %% % As we have noted above, it is easy to establish the equivalence between 
%% NO CALL NOW %% % Problem (\ref{eq:lp_reg}) and Problem (\ref{eq:lp_reg_homog}).
%% NO CALL NOW %% % We note that the same formulation is also used by Nesterov for solving 
%% NO CALL NOW %% % unconstrained convex problems in relative 
%% NO CALL NOW %% % scale~\cite{nesterov2009unconstrained}; and that we used this form 
%% NO CALL NOW %% % implicitly in our discussion in Sections~\ref{sxn:resultsL1-l1reg} 
%% NO CALL NOW %% % and~\ref{sxn:resultsL1-hyperplane}.)
%% NO CALL NOW %% % We prefer this formulation here because it makes our analysis easier 
%% NO CALL NOW %% % to carry out and our algorithms simpler to present.
%% NO CALL NOW %% % %This work deals with the case when $m \gg n$.  
%% NO CALL NOW %% % Let us denote the feasible region by 
%% NO CALL NOW %% % $\Omega = \{ x \in \mathbb{R}^d \,|\, c^T x = 1\}$; let $\mathcal{X}^*$ be 
%% NO CALL NOW %% % the set of all optimal solutions to (\ref{eq:lp_reg_homog}); and let $x^*$ be 
%% NO CALL NOW %% % an arbitrary optimal solution.
%% NO CALL NOW %% % In addition, let $f(x) = \|A x\|_p$, $f^* = \|A x^*\|_p$, and~let
%% NO CALL NOW %% % \begin{equation*}
%% NO CALL NOW %% %   g(x) = A^T [A x]^{p-1} / \|A x\|_p^{p-1} \in \partial f(x),
%% NO CALL NOW %% % \end{equation*}
%% NO CALL NOW %% % where $([A x]^{p-1})_i = \text{sign}(a_i^T x) |a_i^T x|^{p-1}$ and $a_i$ is 
%% NO CALL NOW %% % the $i$-th row of $A$, $i=1,\ldots,n$. 
%% NO CALL NOW %% % Note that $g(x)^T x = f(x)$; and, for simplicity, we assume that $A$ has 
%% NO CALL NOW %% % full column rank and $c \neq \mathbf{0}$. 
%% NO CALL NOW %% % Our assumptions imply that $\mathcal{X}^*$ is a nonempty and bounded convex 
%% NO CALL NOW %% % set and $f^* > 0$. 
%% NO CALL NOW %% % We use $\mathcal{E}(\xi, E) = \{ x \in \mathbb{R}^d \,|\, x = \xi + E z,\ \|z\|_2=1\}$ 
%% NO CALL NOW %% % to describe an ellipsoid where $E \in \mathbb{R}^{d \times d}$ is a 
%% NO CALL NOW %% % non-singular matrix. 
%% NO CALL NOW %% % The volume of a full-dimensional ellipsoid $\mathcal{E}$ is denoted by 
%% NO CALL NOW %% % $|\mathcal{E}|$. 
%% NO CALL NOW %% % We use $\mathcal{S}(S, t) = \{ x \in \mathbb{R}^d \,|\, S x \leq t \}$ to 
%% NO CALL NOW %% % describe a polytope, where $S \in \mathbb{R}^{s \times d}$ and 
%% NO CALL NOW %% % $t \in \mathbb{R}^{s}$ for some $s \geq d+1$.
%% NO CALL NOW %% 
%% NO CALL NOW %% 
%% NO CALL NOW %% \noindent
%% NO CALL NOW %% In the remainder of this section, we will describe several related 
%% NO CALL NOW %% procedures for computing an $\ell_p$ well-conditioned form of an input 
%% NO CALL NOW %% matrix $A$.
%% NO CALL NOW %% For simplicity, we summarize these results in Table~\ref{tab:l1_cond} for 
%% NO CALL NOW %% the special case $p=1$.
%% NO CALL NOW %% Note, in particular, that although our results in this section hold for 
%% NO CALL NOW %% general $\ell_p$, they improve previous results that were specific 
%% NO CALL NOW %% to~$\ell_1$.
%% NO CALL NOW %% 
%% NO CALL NOW %% \begin{table}
%% NO CALL NOW %%   \centering
%% NO CALL NOW %% %%% CHANGE FOR SODA %%%
%% NO CALL NOW %% %%%   \begin{footnotesize}
%% NO CALL NOW %%   \begin{tabular}{c|cc}
%% NO CALL NOW %%     & time & $\kappa_1$ \\
%% NO CALL NOW %%     \hline
%% NO CALL NOW %%     Clarkson~\cite{Cla05} (Lov{\'a}sz~\cite{lovasz}) & $O(n d^5 \log n)$ & $(d (d+1))^{1/2}$ \\
%% NO CALL NOW %%     Theorem \ref{thm:l1_cond_2n} & $O(n d^3 \log n)$ & $2 d$ \\
%% NO CALL NOW %%     Theorem \ref{thm:l1_cond} & $O(n d^2 \log n)$ & $2 d^2$ \\
%% NO CALL NOW %%     Sohler and Woodruff~\cite{SW11} & $O(n d^2 \log d)$ & $O(d^{3/2} \log^{3/2} d)$ \\
%% NO CALL NOW %%     Theorem \ref{thm:l1_cond_fast} & $O(n d \log n)$ & $O(d^{5/2} \log^{1/2} d)$ \\
%% NO CALL NOW %%     Theorem \ref{thm:basisL1} &  $O(n d \log d)$ & $O(d^{5/2} \log^{5/2} d)$ 
%% NO CALL NOW %%   \end{tabular}
%% NO CALL NOW %% %%% CHANGE FOR SODA %%%
%% NO CALL NOW %% %%%   \end{footnotesize}
%% NO CALL NOW %%   \caption{Comparison of our results and previous results for $\ell_1$ norm conditioning algorithms: running time and conditioning quality.
%% NO CALL NOW %% XXX.  XIANGRUI, DO ANY OF THESE NEED TO BE MODIFIED.
%% NO CALL NOW %% }
%% NO CALL NOW %%   \label{tab:l1_cond}
%% NO CALL NOW %% \end{table}
%% NO CALL NOW %% 
%% NO CALL NOW %% 
%% NO CALL NOW %% \subsection{Improved Ellipsoidal Rounding}
%% NO CALL NOW %% \label{sxn:extensionlpXM-rounding}
%% NO CALL NOW %% 
%% NO CALL NOW %% In this section, we provide a deterministic algorithm to compute a 
%% NO CALL NOW %% $2d$-rounding of a centrally symmetric convex set in $\mathbb{R}^d$ that 
%% NO CALL NOW %% is described by a separation oracle.
%% NO CALL NOW %% Recall the well-known result due to John~\cite{john1948extremum} that for a 
%% NO CALL NOW %% centrally symmetric convex set $\mathcal{C}$, there exists a 
%% NO CALL NOW %% $d^{1/2}$-rounding and that such rounding is given by the L{\"o}wner-John 
%% NO CALL NOW %% (LJ) ellipsoid of $\mathcal{C}$, \emph{i.e.}, the minimal-volume ellipsoid 
%% NO CALL NOW %% containing $\mathcal{C}$. 
%% NO CALL NOW %% However, finding this $d^{1/2}$-rounding is a hard problem. 
%% NO CALL NOW %% To state algorithmic results, suppose that $\mathcal{C}$ is described by a 
%% NO CALL NOW %% separation oracle and that we are provided an ellipsoid $\mathcal{E}_0$ that 
%% NO CALL NOW %% gives an $L$-rounding for some $L \geq 1$. 
%% NO CALL NOW %% In this case, the best known algorithmic result of which we are aware is 
%% NO CALL NOW %% that we can find a $(d(d+1))^{1/2}$-rounding in polynomial time, in 
%% NO CALL NOW %% particular, in $O(d^4 \log L)$ calls to the oracle; 
%% NO CALL NOW %% see Lov{\'a}sz~\cite[Theorem 2.4.1]{lovasz}. 
%% NO CALL NOW %% Here, we follow the same construction, but we show that it is much faster to 
%% NO CALL NOW %% find a (slightly worse) $2d$-rounding.
%% NO CALL NOW %% The proof of this theorem may be found in Appendix~\ref{sxn:app-roundingpf}.
%% NO CALL NOW %% 
%% NO CALL NOW %% %%% CHANGE FOR SODA %%%
%% NO CALL NOW %% \begin{theorem}[Improved Ellipsoidal Rounding 1]
%% NO CALL NOW %% %%% \begin{theorem}
%% NO CALL NOW %%   \label{thm:rounding}
%% NO CALL NOW %%   Given a centrally symmetric convex set $\mathcal{C} \subseteq \mathbb{R}^d$
%% NO CALL NOW %%   centered at the origin and described by a separation oracle, and an ellipsoid
%% NO CALL NOW %%   $\mathcal{E}_0$ centered at the origin such that $\mathcal{E}_0/L
%% NO CALL NOW %%   \subseteq \mathcal{C} \subseteq \mathcal{E}_0$ for some $L \geq 1$, it takes
%% NO CALL NOW %%   at most $3.15 d^2 \log L$ calls to the oracle and additional $O(d^4 \log L)$ 
%% NO CALL NOW %%   time to find a $2d$-rounding of $\mathcal{C}$.
%% NO CALL NOW %% \end{theorem}
%% NO CALL NOW %% 
%% NO CALL NOW %% \noindent
%% NO CALL NOW %% Given this result, the following theorem is easily established.
%% NO CALL NOW %% The proof of this theorem may also be found in 
%% NO CALL NOW %% Appendix~\ref{sxn:app-roundingpf}.
%% NO CALL NOW %% 
%% NO CALL NOW %% %%% CHANGE FOR SODA %%%
%% NO CALL NOW %% \begin{theorem}[Improved Ellipsoidal Rounding 2]
%% NO CALL NOW %% %%% \begin{theorem}
%% NO CALL NOW %% \label{thm:l1_cond_2n}
%% NO CALL NOW %% Given $A \in \mathbb{R}^{n \times d}$ with full column rank and 
%% NO CALL NOW %% $p \in [1,\infty]$, it takes at most $O(n d^3 \log n)$ time to find a 
%% NO CALL NOW %% non-singular matrix $R \in \mathbb{R}^{d \times d}$ such that
%% NO CALL NOW %%   \begin{equation*}
%% NO CALL NOW %%     \|y\|_2 \leq \|A \RR y\|_p \leq 2 d \|y\|_2, \quad \forall y \in \mathbb{R}^d.
%% NO CALL NOW %%   \end{equation*}
%% NO CALL NOW %% \end{theorem}
%% NO CALL NOW %% 
%% NO CALL NOW %% \noindent\textbf{Remark.} 
%% NO CALL NOW %% %\paragraph{Remark.} 
%% NO CALL NOW %% Although slightly worse in terms of rounding quality than the well-known 
%% NO CALL NOW %% polynomial time algorithm that computes a $(d (d+1))^{1/2}$-rounding, our 
%% NO CALL NOW %% algorithm is much faster, and it permits us to improves the 
%% NO CALL NOW %% $O(n d^5 \log n)$-time algorithm used by Clarkson~\cite{Cla05} and 
%% NO CALL NOW %% Dasgupta et al.~\cite{DDHKM09_lp_SICOMP}.
%% NO CALL NOW %% In particular, both the algorithm of Clarkson~\cite{Cla05} for $\ell_1$ 
%% NO CALL NOW %% regression as well as the algorithm of Dasgupta 
%% NO CALL NOW %% \emph{et al.}~\cite{DDHKM09_lp_SICOMP} for $\ell_p$ regression take 
%% NO CALL NOW %% $O(n d^5 \log n)$ time to compute an $O(d)$-conditioning.
%% NO CALL NOW %% The $O(n d^3 \log n)$ running time of Theorem~\ref{thm:l1_cond_2n} improves
%% NO CALL NOW %% both of their results to $O(n d^3 \log n)$ running time.
%% NO CALL NOW %% 
%% NO CALL NOW %% \subsection{Improved One-pass Conditioning}
%% NO CALL NOW %% \label{sxn:extensionlpXM-onepasscond}
%% NO CALL NOW %% 
%% NO CALL NOW %% In this section, we use the fast rounding algorithm from 
%% NO CALL NOW %% Section~\ref{sxn:extensionlpXM-rounding} to construct two related 
%% NO CALL NOW %% ``one-pass conditioning'' algorithms for $\ell_p$ regression. 
%% NO CALL NOW %% Our algorithms work for general $p \in [1, \infty]$, while being competitive 
%% NO CALL NOW %% with or even better than special-purpose conditioning algorithms such as 
%% NO CALL NOW %% those developed by Sohler and Woodruff~\cite{SW11} and by us in 
%% NO CALL NOW %% Section~\ref{sxn:resultsL1} for $\ell_1$ regression.
%% NO CALL NOW %% The motivation for our one-pass conditioning algorithm is that, although 
%% NO CALL NOW %% by the results of Section~\ref{sxn:extensionlpXM-rounding} we can find a 
%% NO CALL NOW %% $2d$-rounding much faster than a $(d(d+1))^{1/2}$-rounding, it is still not 
%% NO CALL NOW %% immediately applicable to very large-scale $\ell_1$ or $\ell_p$ regression 
%% NO CALL NOW %% problems, because each call to the oracle requires a pass over the data. 
%% NO CALL NOW %% 
%% NO CALL NOW %% To develop our one-pass conditioning algorithm, we could group $d$ calls 
%% NO CALL NOW %% together within a single pass, but we would still need $O(d \log n)$ passes. 
%% NO CALL NOW %% In order to balance the cost-performance trade-off, we present a one-pass 
%% NO CALL NOW %% conditioning algorithm that gives a $2 d^{2/p}$-conditioning of $A$.
%% NO CALL NOW %% Details are provided in the \textsf{OnePassConditioning} algorithm in 
%% NO CALL NOW %% Figure~\ref{alg:l1_cond}.
%% NO CALL NOW %% The \textsf{OnePassConditioning} algorithm takes as input a full column-rank 
%% NO CALL NOW %% matrix $A\in \mathbb{R}^{n \times d}$ and a number $p \in [1, 2)$; and it
%% NO CALL NOW %% returns as out a non-singular matrix $E \in \mathbb{R}^{d \times d}$.
%% NO CALL NOW %% Note that it is a deterministic algorithm.
%% NO CALL NOW %% The following is our main theorem for the \textsf{OnePassConditioning} 
%% NO CALL NOW %% algorithm.
%% NO CALL NOW %% The proof of this theorem may be found in Appendix~\ref{sxn:app-onepasspf}.
%% NO CALL NOW %% 
%% NO CALL NOW %% \input{alg-LpCond1}
%% NO CALL NOW %% 
%% NO CALL NOW %% %%% CHANGE FOR SODA %%%
%% NO CALL NOW %% \begin{theorem}[One-pass Conditioning]
%% NO CALL NOW %% %%% \begin{theorem}
%% NO CALL NOW %% Let $A$ be a full rank $n \times d$ matrix, with $n > d$, and let $p\in[1,2)$.
%% NO CALL NOW %% Then, there exists an algorithm (the \textsf{OnePassConditioning} 
%% NO CALL NOW %% algorithm of Figure~\ref{alg:l1_cond}) 
%% NO CALL NOW %% that runs in time $O(nd^2\log n)$ and
%% NO CALL NOW %% that returns as output a
%% NO CALL NOW %% non-singular matrix $E \in \mathbb{R}^{d \times d}$ such that
%% NO CALL NOW %% $ \kappa_p(A E) \le 2 d^{2/p}$, \emph{i.e.}, such that
%% NO CALL NOW %% $$
%% NO CALL NOW %% \|y\|_2 \leq \|A E y\|_p \leq 2 d^{2/p} \|y\|_2,\ \forall y \in \mathbb{R}^d.
%% NO CALL NOW %% $$
%% NO CALL NOW %% \label{thm:l1_cond}
%% NO CALL NOW %% \end{theorem}
%% NO CALL NOW %% 
%% NO CALL NOW %% \noindent\textbf{Remark.} 
%% NO CALL NOW %% %\paragraph{Remark.} 
%% NO CALL NOW %% Note that the rounding procedure is
%% NO CALL NOW %% applied to a problem of size $M d \times d \approx n/d \times d$. 
%% NO CALL NOW %% Therefore,
%% NO CALL NOW %% the \textsf{OnePassConditioning} algorithm only needs a single pass to the 
%% NO CALL NOW %% data with
%% NO CALL NOW %% $O(n d^2)$ FLOPs and an offline work of $O((n d^2 + d^4) \log n)$ FLOPs. 
%% NO CALL NOW %% The offline work requires $n$ RAM, which might be too much for
%% NO CALL NOW %% large-scale problems. In such case, we can increase the block size from $d^2$
%% NO CALL NOW %% to, for example, $d^3$. It gives us a $2 d^{3/p - 1/2}$-conditioning algorithm
%% NO CALL NOW %% that only needs $n/d$ offline RAM and $O((n d + d^4) \log n)$ offline
%% NO CALL NOW %% FLOPs. The proof follows similar arguments. 
%% NO CALL NOW %% Although the online work remains $O(n d^2)$, it is embarrassingly parallel.
%% NO CALL NOW %% %%% and can be well distributed
%% NO CALL NOW %% %%% on MapReduce-like environments.
%% NO CALL NOW %% 
%% NO CALL NOW %% \noindent\textbf{Remark.} 
%% NO CALL NOW %% %\paragraph{Remark.} 
%% NO CALL NOW %% For large-scale strongly over-determined problems, the 
%% NO CALL NOW %% \textsf{OnePassConditioning} algorithm described below, with block size 
%% NO CALL NOW %% roughly $d^3$ seems to be a good compromise in practice.
%% NO CALL NOW %% This guarantees $2 d^{3/p-1/2}$-conditioning (with no hidden constants), 
%% NO CALL NOW %% and the $O(n d^2)$ online work can be easily distributed in MapReduce-like
%% NO CALL NOW %% environments.
%% NO CALL NOW %% 
%% NO CALL NOW %% Finally, as a matter of theoretical interest, we can also improve the online 
%% NO CALL NOW %% FLOPs to $O(n d \log d)$ by replacing the SVD of each submatrix by a FJLT
%% NO CALL NOW %% that preserves the $\ell_2$-norm distances (up to a constant factor) of an 
%% NO CALL NOW %% entire subspace of vectors.
%% NO CALL NOW %% It results an $O(d^{3/p-1/2} \log^{1/p-1/2} d)$-conditioning algorithm that 
%% NO CALL NOW %% needs $O(n d \log d)$ online FLOPs, $O(n / d)$ offline RAM, and 
%% NO CALL NOW %% $O((n d + d^4) \log n)$ offline FLOPs. 
%% NO CALL NOW %% Details are provided in the \textsf{FasterOnePassConditioning} algorithm 
%% NO CALL NOW %% in Figure~\ref{alg:l1_cond_fast}.
%% NO CALL NOW %% The \textsf{OnePassConditioning} algorithm takes as input a full column-rank 
%% NO CALL NOW %% matrix $A\in \mathbb{R}^{n \times d}$ and a number $p \in [1, 2)$; and it
%% NO CALL NOW %% returns as out a non-singular matrix $E \in \mathbb{R}^{d \times d}$.
%% NO CALL NOW %% Note that because of the FJLT, this is a randomized algorithm.
%% NO CALL NOW %% The following is our main theorem for the \textsf{FasterOnePassConditioning} 
%% NO CALL NOW %% algorithm.
%% NO CALL NOW %% The proof of this theorem may also be found in 
%% NO CALL NOW %% Appendix~\ref{sxn:app-onepasspf}.
%% NO CALL NOW %% 
%% NO CALL NOW %% \input{alg-LpCond2}
%% NO CALL NOW %% 
%% NO CALL NOW %% %%% CHANGE FOR SODA %%%
%% NO CALL NOW %% \begin{theorem}[Faster One-pass Conditioning]
%% NO CALL NOW %% %%% \begin{theorem}
%% NO CALL NOW %% Let $A$ be a full rank $n \times d$ matrix, with $n > d$, and let $p\in[1,2)$.
%% NO CALL NOW %% Then, there exists an algorithm (the \textsf{FasterOnePassConditioning} 
%% NO CALL NOW %% algorithm of Figure~\ref{alg:l1_cond_fast}) 
%% NO CALL NOW %% that runs in time $O(nd\log n)$ and that returns as output a
%% NO CALL NOW %% non-singular matrix $E \in \mathbb{R}^{d \times d}$ such that
%% NO CALL NOW %% $ \kappa_p(A E) \leq O(d^{3/p-1/2} \log^{1/p-1/2} d) $, \emph{i.e.}, such that
%% NO CALL NOW %% $$
%% NO CALL NOW %% \|y\|_2 \leq \|A E y\|_p 
%% NO CALL NOW %% \leq  O(d^{3/p-1/2} \log^{1/p-1/2} d)  \|y\|_2,\ \forall y \in \mathbb{R}^d.
%% NO CALL NOW %% $$
%% NO CALL NOW %% \label{thm:l1_cond_fast}
%% NO CALL NOW %% \end{theorem}
%% NO CALL NOW %% 
%% NO CALL NOW %% \noindent\textbf{Remark.} 
%% NO CALL NOW %% %\paragraph{Remark.} 
%% NO CALL NOW %% Although we are interested in $p \in [1, 2)$, it is easy to see that our 
%% NO CALL NOW %% approach works for all $p \in [1, \infty]$. For the case when $p=1$, Sohler 
%% NO CALL NOW %% and Woodruff~\cite{SW11} propose a Cauchy transform 
%% NO CALL NOW %% $\Pi \in \mathbb{R}^{O(d \log d) \times n}$ such that
%% NO CALL NOW %% \begin{equation*}
%% NO CALL NOW %%   \|\Pi A x\|_1 \leq \|A x\|_1 \leq O(d \log d) \|\Pi A x\|_1, \quad \forall x \in \mathbb{R}^d.
%% NO CALL NOW %% \end{equation*}
%% NO CALL NOW %% The running time is $O(n d^2 \log d)$.  Let $R$ be the $R$ matrix of
%% NO CALL NOW %% the QR factorization of $\Pi A$. We have, 
%% NO CALL NOW %% \begin{align*}
%% NO CALL NOW %%   \|R x\|_2 &= \|\Pi A x\|_2 \leq \|\Pi A x\|_1 \leq \|A x\|_1 \\
%% NO CALL NOW %%   &\leq O(d \log d) \|\Pi A x\|_1 \leq O(d^{3/2} \log^{3/2} d) \|\Pi A x\|_2 \\
%% NO CALL NOW %%   &\leq O(d^{3/2} \log^{3/2} d) \| R x \|_2, \quad \forall x \in \mathbb{R}^d.
%% NO CALL NOW %% \end{align*}
%% NO CALL NOW %% Hence $\kappa_1(A R^{-1}) = O(d^{3/2} \log^{3/2} d)$. 
%% NO CALL NOW %% Our FCT2 computes a $\tilde{\Pi} \in \mathbb{R}^{O(d \log d) \times m}$ 
%% NO CALL NOW %% in $O(n d \log d)$ time such~that
%% NO CALL NOW %% \begin{equation*}
%% NO CALL NOW %%   \|\tilde{\Pi} A x\|_1 \leq \|A x\|_1 \leq O(d^2 \log^2 d) \|\tilde{\Pi} A x\|_1, \quad \forall x \in \mathbb{R}^d.
%% NO CALL NOW %% \end{equation*}
%% NO CALL NOW %% This leads to an $O(d^{5/2} \log^{5/2} d)$-conditioning algorithm. 
%% NO CALL NOW %% 

